Fixed-point equations solving Risk-sensitive MDP with constraint

There are no computationally feasible algorithms that provide solutions to the finite horizon Risk-sensitive Constrained Markov Decision Process (Risk-CMDP) problem, even for problems with moderate horizon. With an aim to design the same, we derive a fixed-point equation such that the optimal policy of Risk-CMDP is also a solution. We further provide two optimization problems equivalent to the Risk-CMDP. These formulations are instrumental in designing a global algorithm that converges to the optimal policy. The proposed algorithm is based on random restarts and a local improvement step, where the local improvement step utilizes the solution of the derived fixed-point equation; random restarts ensure global optimization. We also provide numerical examples to illustrate the feasibility of our algorithm for inventory control problem with risk-sensitive cost and constraint. The complexity of the algorithm grows only linearly with the time-horizon.

==> arxive_ACC Risk sensitive constrained MDP/bibliography.tex <==

\begin{thebibliography}{}
\bibitem{puterman}
Puterman, Martin L. Markov decision processes: discrete stochastic dynamic programming. John Wiley \& Sons, 2014.

\bibitem{Jaquette73}
Jaquette, Stratton C. "Markov decision processes with a new optimality criterion: Discrete time." The Annals of Statistics 1.3 (1973): 496-505.

\bibitem{inv}
Chen X, Sim M, Simchi-Levi D, Sun P. Risk aversion in inventory management. Operations Research. 2007 Oct;55(5):828-42.

\bibitem{Jaquette76}
Jaquette, Stratton C. "A utility criterion for Markov decision processes." Management Science 23.1 (1976): 43-49.

\bibitem{avgg}
Di Masi, Giovanni B., and Lukasz Stettner. "Risk-sensitive control of discrete-time Markov processes with infinite horizon." SIAM Journal on Control and Optimization 38.1 (1999): 61-78.
\bibitem{usto}
Coraluppi, Stefano P., and Steven I. Marcus. "Risk-sensitive and minimax control of discrete-time, finite-state Markov decision processes." Automatica 35.2 (1999): 301-309.

\bibitem{uday_uss}
Kumar M, Uday, et al. "Ultimately Stationary Policies to Approximate Risk-Sensitive Discounted MDPs." Proceedings of the 12th EAI International Conference on Performance Evaluation Methodologies and Tools. 2019.

\bibitem{Howard}
Howard, Ronald A., and James E. Matheson. "Risk-sensitive Markov decision processes." Management science 18.7 (1972): 356-369.

\bibitem{atul}
Kumar, Atul, Veeraruna Kavitha, and Nandyala Hemachandra. "Finite horizon risk sensitive MDP and linear programming." 2015 54th IEEE Conference on Decision and Control (CDC). IEEE, 2015.

\bibitem{uday}
Kumar M, Uday, et al.
"Approximate Solutions To Constrained Risk-Sensitive Markov Decision Processes." 
European Journal of Operational Research (2023). Also available at \href{http://arxiv.org/abs/2209.14963}{http://arxiv.org/abs/2209.14963}

\bibitem{sim_annealing}
Bertsimas, Dimitris, and John Tsitsiklis. "Simulated annealing." Statistical science 8.1 (1993): 10-15.


\bibitem{global}Pepelyshev, Andrey, Anatoly Zhigljavsky, and Antanas Žilinskas. "Performance of global random search algorithms for large dimensions." Journal of Global Optimization 71.1 (2018): 57-71.

\bibitem{kushner2003stochastic}
Kushner, Harold, and G. George Yin. Stochastic approximation and recursive algorithms and applications. Vol. 35. Springer Science 
\& Business Media, 2003.

\bibitem{eitan}
Altman, Eitan. Constrained Markov decision processes: stochastic modeling. Routledge, 1999.
% \bibitem{TR}
% {\color{red}Technical report, arxive}

\TR{\bibitem{TR}
Singh, Vartika, and Veeraruna Kavitha. "Fixed-point equations solving Risk-sensitive MDP with constraint." arXiv preprint arXiv:2210.02686 (2022).}{}
\end{thebibliography}
